To Transfer or Not to Transfer: Misclassification Attacks Against Transfer Learned Text Classifiers

Transfer learning --- transferring learned knowledge --- has brought a paradigm shift in the way models are trained. The lucrative benefits of improved accuracy and reduced training time have shown promise in training models with constrained computational resources and fewer training samples. Specifically, publicly available text-based models such as GloVe and BERT that are trained on large corpus of datasets have seen ubiquitous adoption in practice. In this paper, we ask, "can transfer learning in text prediction models be exploited to perform misclassification attacks?" As our main contribution, we present novel attack techniques that utilize unintended features learnt in the teacher (public) model to generate adversarial examples for student (downstream) models. To the best of our knowledge, ours is the first work to show that transfer learning from state-of-the-art word-based and sentence-based teacher models increase the susceptibility of student models to misclassification attacks. First, we propose a novel word-score based attack algorithm for generating adversarial examples against student models trained using context-free word-level embedding model. On binary classification tasks trained using the GloVe teacher model, we achieve an average attack accuracy of 97% for the IMDB Movie Reviews and 80% for the Fake News Detection. For multi-class tasks, we divide the Newsgroup dataset into 6 and 20 classes and achieve an average attack accuracy of 75% and 41% respectively. Next, we present length-based and sentence-based misclassification attacks for the Fake News Detection task trained using a context-aware BERT model and achieve 78% and 39% attack accuracy respectively. Thus, our results motivate the need for designing training techniques that are robust to unintended feature learning, specifically for transfer learned models.

==> images/poison.tex <==
%% This file was created by tikzplotlib v0.8.4.
%\begin{tikzpicture}[scale=0.85]
%
%\begin{axis}[
%tick align=outside,
%tick pos=left,
%x grid style={white!69.01960784313725!black},
%xlabel={Epochs},
%xmin=0.3, xmax=15.7,
%xtick style={color=black},
%y grid style={white!69.01960784313725!black},
%ylabel={Softmax Probability of Poisoned News},
%ymin=-1.1, ymax=1.1,
%ytick style={color=black}
%]
%\path [fill=white, fill opacity=0.5]
%(axis cs:1,1)
%--(axis cs:1,0)
%--(axis cs:2,0)
%--(axis cs:3,0)
%--(axis cs:4,0)
%--(axis cs:5,0)
%--(axis cs:6,0)
%--(axis cs:7,0)
%--(axis cs:8,0)
%--(axis cs:9,0)
%--(axis cs:10,0)
%--(axis cs:11,0)
%--(axis cs:12,0)
%--(axis cs:13,0)
%--(axis cs:14,0)
%--(axis cs:15,0)
%--(axis cs:15,1)
%--(axis cs:15,1)
%--(axis cs:14,1)
%--(axis cs:13,1)
%--(axis cs:12,1)
%--(axis cs:11,1)
%--(axis cs:10,1)
%--(axis cs:9,1)
%--(axis cs:8,1)
%--(axis cs:7,1)
%--(axis cs:6,1)
%--(axis cs:5,1)
%--(axis cs:4,1)
%--(axis cs:3,1)
%--(axis cs:2,1)
%--(axis cs:1,1)
%--cycle;
%
%\path [fill=white, fill opacity=0.5]
%(axis cs:1,-1)
%--(axis cs:1,0)
%--(axis cs:2,0)
%--(axis cs:3,0)
%--(axis cs:4,0)
%--(axis cs:5,0)
%--(axis cs:6,0)
%--(axis cs:7,0)
%--(axis cs:8,0)
%--(axis cs:9,0)
%--(axis cs:10,0)
%--(axis cs:11,0)
%--(axis cs:12,0)
%--(axis cs:13,0)
%--(axis cs:14,0)
%--(axis cs:15,0)
%--(axis cs:15,-1)
%--(axis cs:15,-1)
%--(axis cs:14,-1)
%--(axis cs:13,-1)
%--(axis cs:12,-1)
%--(axis cs:11,-1)
%--(axis cs:10,-1)
%--(axis cs:9,-1)
%--(axis cs:8,-1)
%--(axis cs:7,-1)
%--(axis cs:6,-1)
%--(axis cs:5,-1)
%--(axis cs:4,-1)
%--(axis cs:3,-1)
%--(axis cs:2,-1)
%--(axis cs:1,-1)
%--cycle;
%
%\addplot [semithick, blue!54.509803921568626!black, mark=asterisk, mark size=3, mark options={solid}]
%table {%
%1 -0.931442257101942
%2 -0.977083672663538
%3 -0.974900067496047
%4 -0.514920274077965
%5 0.93402665884497
%6 0.940703475867907
%7 0.989609242861068
%8 0.759906136491178
%9 0.820653547283915
%10 0.989581638122229
%11 0.997700002420134
%12 0.987966804788376
%13 0.991514412300335
%14 0.987250993316035
%15 0.981645879904174
%};\label{plot_one}
%\addplot [semithick, red!54.509803921568626!black, mark=triangle*, mark size=3, mark options={solid}]
%table {%
%1 0.999996662145463
%2 1
%3 1
%4 1
%5 0.990603526475645
%6 0.999996662145463
%7 0.569988601876171
%8 0.830575585879893
%9 0.821968842054047
%10 0.997104790884505
%11 0.614797908522248
%12 0.998550750960449
%13 0.98759965113555
%14 0.995030394922902
%15 0.9771354951632
%};\label{plot_two}
%\addplot [semithick, green!39.21568627450981!black, mark=*, mark size=3, mark options={solid}]
%table {%
%1 -0.893504291622422
%2 -0.991977382660138
%3 -0.999786399768903
%4 -0.998459573144821
%5 -0.99577487551399
%6 -0.999154924995685
%7 -0.997564425609031
%8 -0.98993442328998
%9 -0.993120837395231
%10 -0.991271663886049
%11 -0.98784197136548
%12 -0.998227500089597
%13 -0.993382985742066
%14 -0.995802415597607
%15 -0.997812997171324
%};\label{plot_three}
%\addplot [semithick, black]
%table {%
%1 0
%2 0
%3 0
%4 0
%5 0
%6 0
%7 0
%8 0
%9 0
%10 0
%11 0
%12 0
%13 0
%14 0
%15 0
%};
%\node at (axis cs:10,-0.5)[
%  scale=0.8,
%  anchor=base west,
%  text=black,
%  rotate=0.0
%]{FAKE};
%\node at (axis cs:10,0.5)[
%  scale=0.8,
%  anchor=base west,
%  text=black,
%  rotate=0.0
%]{REAL};
%\end{axis}
%
%\begin{axis}[
%axis y line=right,
%tick align=outside,
%x grid style={white!69.01960784313725!black},
%xmin=0.3, xmax=15.7,
%xtick pos=left,
%xtick style={color=black},
%y grid style={white!69.01960784313725!black},
%ylabel={Model Accuracy},
%ymin=0.4633, ymax=0.9627,
%legend columns=2,
%legend style={at={(0.5,-0.25)},anchor=north},
%ytick pos=right,
%ytick style={color=black}
%]
%\addplot [semithick, blue, dash pattern=on 1pt off 3pt on 3pt off 3pt]
%table {%
%1 0.724
%2 0.486
%3 0.791
%4 0.599
%5 0.793
%6 0.869
%7 0.905
%8 0.901
%9 0.919
%10 0.911
%11 0.932
%12 0.94
%13 0.932
%14 0.921
%15 0.923
%};\label{plot_four}
%\addplot [semithick, red, dotted]
%table {%
%1 0.704
%2 0.734
%3 0.828
%4 0.82
%5 0.828
%6 0.8
%7 0.82
%8 0.848
%9 0.875
%10 0.87
%11 0.876
%12 0.879
%13 0.881
%14 0.91
%15 0.92
%};\label{plot_five}
%\addplot [semithick, green!50.19607843137255!black, dashed]
%table {%
%1 0.63
%2 0.794
%3 0.826
%4 0.825
%5 0.823
%6 0.816
%7 0.841
%8 0.864
%9 0.891
%10 0.908
%11 0.892
%12 0.919
%13 0.925
%14 0.921
%15 0.925
%};\label{plot_six}
%
%\addlegendimage{/pgfplots/refstyle=plot_one}\addlegendentry{Prob Poision}
%\addlegendimage{/pgfplots/refstyle=plot_two}\addlegendentry{Prob Poision-2}
%\addlegendimage{/pgfplots/refstyle=plot_three}\addlegendentry{Prob Original}
%\addlegendimage{/pgfplots/refstyle=plot_four}\addlegendentry{Acc Poision}
%\addlegendimage{/pgfplots/refstyle=plot_five}\addlegendentry{Acc Poision-2}
%\addlegendimage{/pgfplots/refstyle=plot_six}\addlegendentry{Acc Original}
%\end{axis}
%
%\end{tikzpicture}

% This file was created by tikzplotlib v0.8.4.
\begin{tikzpicture}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xlabel={Epochs},
xmin=0.3, xmax=15.7,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Softmax Probability of Poisoned News},
ymin=-1.1, ymax=1.1,
ytick style={color=black}
]
\path [fill=white, fill opacity=0.5]
(axis cs:1,1)
--(axis cs:1,0)
--(axis cs:2,0)
--(axis cs:3,0)
--(axis cs:4,0)
--(axis cs:5,0)
--(axis cs:6,0)
--(axis cs:7,0)
--(axis cs:8,0)
--(axis cs:9,0)
--(axis cs:10,0)
--(axis cs:11,0)
--(axis cs:12,0)
--(axis cs:13,0)
--(axis cs:14,0)
--(axis cs:15,0)
--(axis cs:15,1)
--(axis cs:15,1)
--(axis cs:14,1)
--(axis cs:13,1)
--(axis cs:12,1)
--(axis cs:11,1)
--(axis cs:10,1)
--(axis cs:9,1)
--(axis cs:8,1)
--(axis cs:7,1)
--(axis cs:6,1)
--(axis cs:5,1)
--(axis cs:4,1)
--(axis cs:3,1)
--(axis cs:2,1)
--(axis cs:1,1)
--cycle;

\path [fill=white, fill opacity=0.5]
(axis cs:1,-1)
--(axis cs:1,0)
--(axis cs:2,0)
--(axis cs:3,0)
--(axis cs:4,0)
--(axis cs:5,0)
--(axis cs:6,0)
--(axis cs:7,0)
--(axis cs:8,0)
--(axis cs:9,0)
--(axis cs:10,0)
--(axis cs:11,0)
--(axis cs:12,0)
--(axis cs:13,0)
--(axis cs:14,0)
--(axis cs:15,0)
--(axis cs:15,-1)
--(axis cs:15,-1)
--(axis cs:14,-1)
--(axis cs:13,-1)
--(axis cs:12,-1)
--(axis cs:11,-1)
--(axis cs:10,-1)
--(axis cs:9,-1)
--(axis cs:8,-1)
--(axis cs:7,-1)
--(axis cs:6,-1)
--(axis cs:5,-1)
--(axis cs:4,-1)
--(axis cs:3,-1)
--(axis cs:2,-1)
--(axis cs:1,-1)
--cycle;

\addplot [semithick, red!54.509803921568626!black, mark=asterisk, mark size=3, mark options={solid}]
table {%
1 -0.931442257101942
2 -0.977083672663538
3 -0.974900067496047
4 -0.514920274077965
5 0.93402665884497
6 0.940703475867907
7 0.989609242861068
8 0.759906136491178
9 0.820653547283915
10 0.989581638122229
11 0.997700002420134
12 0.987966804788376
13 0.991514412300335
14 0.987250993316035
15 0.981645879904174
};
\addplot [semithick, green!39.21568627450981!black, mark=*, mark size=3, mark options={solid}]
table {%
1 -0.893504291622422
2 -0.991977382660138
3 -0.999786399768903
4 -0.998459573144821
5 -0.99577487551399
6 -0.999154924995685
7 -0.997564425609031
8 -0.98993442328998
9 -0.993120837395231
10 -0.991271663886049
11 -0.98784197136548
12 -0.998227500089597
13 -0.993382985742066
14 -0.995802415597607
15 -0.997812997171324
};\label{plot_one}
\addplot [semithick, black]
table {%
1 0
2 0
3 0
4 0
5 0
6 0
7 0
8 0
9 0
10 0
11 0
12 0
13 0
14 0
15 0
};\label{plot_two}
\node at (axis cs:10,-0.5)[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{FAKE};
\node at (axis cs:10,0.5)[
  scale=0.5,
  anchor=base west,
  text=black,
  rotate=0.0
]{REAL};
\end{axis}

\begin{axis}[
axis y line=right,
tick align=outside,
x grid style={white!69.01960784313725!black},
xmin=0.3, xmax=15.7,
xtick pos=left,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Model Accuracy},
ymin=0.4633, ymax=0.9627,
legend columns=2,
legend style={at={(0.5,-0.25)},anchor=north},
ytick pos=right,
ytick style={color=black}
]
\addplot [semithick, red, dash pattern=on 1pt off 3pt on 3pt off 3pt]
table {%
1 0.724
2 0.486
3 0.791
4 0.599
5 0.793
6 0.869
7 0.905
8 0.901
9 0.919
10 0.911
11 0.932
12 0.94
13 0.932
14 0.921
15 0.923
};\label{plot_three}
\addplot [semithick, green!50.19607843137255!black, dashed]
table {%
1 0.63
2 0.794
3 0.826
4 0.825
5 0.823
6 0.816
7 0.841
8 0.864
9 0.891
10 0.908
11 0.892
12 0.919
13 0.925
14 0.921
15 0.925
};\label{plot_four}

\addlegendimage{/pgfplots/refstyle=plot_one}\addlegendentry{Acc Poision}
\addlegendimage{/pgfplots/refstyle=plot_two}\addlegendentry{Acc Original}
\addlegendimage{/pgfplots/refstyle=plot_three}\addlegendentry{Prob Poision}
\addlegendimage{/pgfplots/refstyle=plot_four}\addlegendentry{Prob Original}

\end{axis}

\end{tikzpicture}

==> overview.tex <==
\section{Overview}

\shruti{Relate the below paragraph to the terms used the word-level embedding and sentence-level embedding from Section 2.}
In the previous section, we briefly introduced the attacks considered in the transfer learned setting - Adversarial attack and Poisoning attack. We consider both of these attacks in two different transfer learned setting- word level knowledge transfer via word embedding and sentence level knowledge transfer via sentence embedding. The two setting are different; the student model takes the input in form of words when trained using word embedding representation, while the sentence embedding trained student model takes the vector representation of whole text data as the input to model. If the input x consists of words $w_1 \ldots w_n$, then the T(x) actually comprises of T($w_1$) .. T($w_n$). Thus, the classification output of the student model is directly dependent on the words present in the input sentence. The sentence embeddings on other hand directly inputs T(x) to the student model. Therefore, the student model never directly learns what words were present in the input; it is more dependent on how whether T(x) carries the information of the words. The output of the student model is thus more dependent on the features extracted by the teacher sentence embedding than word embeddings as the relationship between words and other features are learn by the student model itself using the training dataset. 

\paragraph{Key Insight: Learning Unintended Features.}
Although our attack strategies are different for different transfer learned setting, they are however based on the common theme of models making predictions based on unintended features. The whole idea of neural network based models is that it doesn't alleviates the requirement of feature extraction, or the process of extracting the features from the dataset on which the predictions should be based. On one hand, removing this tedious human task has lead to unprecedented growth in the area of artificial intelligence with models achieving massive boost in accuracy with large amount of data. On the other hand, this had lead to the whole areas of research on trying to understand based on which features these models are making predictions. The neural network learns the required features from the training dataset that leads to highest performance accuracy but it has also lead the models to make predictions based on unintended features. Recent papers have shown that deep learning models often make prediction not undesirable features like race, gender etc, which leads to the question of trying to make these models fair and unbiased. But this still doesn't answer the question of whether these models are making predictions based on the correct features. In this work, we show empirically how these text classification models make predictions based on features that doesn't capture the task intended to perform by the model. While, these biases are present in the training dataset, it is not the intended features for the task. For example, while certain words like 'Wikileaks', 'Sources' etc are more common in fake news than in real news, classifying news based on presence of certain words is not what is expected out of news classification models. It maybe argued that if the training dataset contains this bias then maybe it is indeed an important feature for classifying news. This argument is true if the test dataset also follows the same distribution of words, but the distribution of words is user dependent and therefore can be maliciously changed to fool the model. In this paper, we present attacks that exploits these unintended features learned by the models, either from the teacher models or the children model itself. 
\shruti{May be give example of length as the unintended feature as well?}

\shruti{Think of a better name for this paragraph}

\paragraph{Adversarial examples}
We consider a text binary classification setting consisting of input-label pairs $(x,y) \in T \times \{+1,-1\}$ from distribution D. The objective is to learn a classifier $C: T \rightarrow \{+1,-1\}$, that takes an input text x drawn from $T$ and maps it to label y belonging to set $\{+1,-1\}$. An feature is defined as a function $f$ can takes a input x from $T$ and maps it to an n-dimensional vector $R$, $f:T \rightarrow R$. 

A classifier thus can be defined as $C= (F,w,b)$ where F comprises of a set of feature, w is a weight vector and b is a bias value.  Thus for an input x, the classifier will then make prediction based on the dot product between feature f belonging to set F and corresponding weight $w_f$ associated to them. 

\begin{equation}
  C(x)=\left\{
  \begin{array}{@{}ll@{}}
    +1, & \text{if}\ \sum_{f \in F} w_f \cdot f(x) + b > 0 \\
    -1, & \text{otherwise}
  \end{array}\right.
\end{equation}

In a recent work, Ilyas et al. \cite{ilyas2019adversarial} divided the feature set F into primarily two categories based on where the feature is robust or non-robust. We extend this these classifications to text setting and describe why it is different from image-based features.  

%\begin{itemize}
% \item \boldmath$\rho-$\textbf{useful feature}: A feature f is called $\rho$ useful if it is correlated to the true label such that \newline
% $E_{(x,y) \sim D} [y \cdot f(x)] \geq \rho$
% 
% \item \boldmath$\gamma-$\textbf{robust useful feature}: A feature f is called $\gamma$ robust useful if it is $\gamma$ useful after adding adversarial perturbation $\delta$ from valid perturbations $\Delta$, i.e. \newline
% $E_{(x,y) \sim D} [\min_{\delta \in \Delta} y \cdot f(x+\delta)] \geq \gamma$
% 
% \item \textbf{Useful, non-robust features}: This refers to a feature that is $\rho-$useful for some $rho$ much greater than zero but is not  $\gamma$ robust against adversarial perturbation for $\gamma>0$. These features will lead to increase in test accuracy but will be susceptible to adversarial perturbations.  
%\end{itemize}

Perturbation can be defined as adversarial changes that doesn't change the semantic structure of the input. This raises the question of what comprises adversarial changes? To answer this question, we need to look into our threat model. An adversarial change is dependent on the manipulative power of the attacker. While in case of images, the common threat model, Adversarial attack, assumes that attacker can make small modification to the input image such that $L_p$ distance between images is less than a given threshold $th$. Recently, the community has started exploring more powerful threat model, where adversary can make random translation to image\cite{}, or insert random object inside images \cite{}. These attacks are often known as corruption attacks. However, the main idea to define set of valid perturbations $\Delta$ in a given threat model.

 In the case of text, it is more difficult to quantify the semantic similarity of input. We assume the attacker can write a sentence with any valid English word and the Although, prior works considers the threshold value $th$ to be the fraction of words replaced in an input.  But, there is something fundamentally missing about these assumptions. Let us consider an image classification task where we want to figure out if there are any black pixels in the image. Thus, given an input x with no black pixels, the model outputs label corresponding to no black pixels. Let's add an adversarial perturbation $\delta' \in \Delta$ of changing a pixel to black, which flips the label prediction. However, this is an indented feature as the model is trying to detect black pixel. Similarly, in sentiment analysis flipping a positive sentiment word to negative flips the classification of model, however this is a desired feature. 

 We, therefore, claim that valid perturbations are dependent on the classification tasks. It shouldn't depend on similarity measured by $L_p$ distance in images or fraction of replaced words in case of text inputs. We define a valid perturbation to be any change to the input that is independent of the task. In an image classification task of human face recognization, adding a spectacle to the face is considered a valid perturbation as it is independent of the task. This change may result in a large $L_p$ distance between actual input and adversarial input. Similarly for text classification for sentiment analysis, adding n number of lines shouldn't change the classification as long as the new sentences express the same sentiment. We, therefore, modify the above classification of features.
 
 \begin{itemize}
 \item \boldmath$\rho-$\textbf{useful feature}: A feature f is called $\rho$ useful if it is correlated to the true label such that \newline
 $E_{(x,y) \sim D} [y \cdot f(x)] \geq \rho$
 
 \item \boldmath$\gamma-$\textbf{intended useful feature}: A feature f is called $\gamma$ robust useful if it is $\gamma$ useful even after adding adversarial change c to generate x' from x,  $c$ belongs to changes not relevant to binary classification task i.e. \newline
 $E_{(x,y) \sim D} [ y \cdot f(x')] \geq \gamma$\newline
 
 \item \textbf{Useful, unintended features}: This refers to a feature that is $\rho-$useful for some $rho$ much greater than zero but is not $\gamma$ intended against adversarial changes for $\gamma>0$. These features refers to biases present in training dataset that may be present in the test dataset leading to high accuracy, but is not the intended feature for the classification task. 
\end{itemize}

 Ilyas et al. \cite{ilyas2019adversarial} discusses how classification models while optimizing for features that increases accuracy can learn from useful, non-robust features, which then leads to models being susceptible to adversarial perturbations. The model optimizes to any signal, that maybe incomprehensible to humans. They call these features to be 'non-robust'. However, the making a classification model robust against any adversarial examples involves learning from only intended features, that may or may not be detectable by humans. In this paper, we show adversarial attacks by exploiting some of the unintended features learned by the student classifiers, that maybe detectable by humans. 

\paragraph{Attack Algorithms}
\shruti{Let us try to give a high-level overview of the rest of the paper in here. Add a section number reference to each of the discussed points. Give a more structured overview with respect to the adversarial \& poisoning attack strategies. Talk about binary \& multi-class attacks. What is our Sentence level embedding attack and the effect of defenses}

Due to the difference in the setting of both transfer learned models, we will show how our attack strategy is also based different features. In case of word embeddings, the words present in input and their representation T(w) plays an important role in classification and are attack strategy exploits this fact. However, the attacks on sentence embedding learned model are dependent on how the output value of the embedding representation of input x, T(x). In the following sections, we therefore explore the attack algorithms in both of these transfer-learned setting and understand how they are different from one other. We will initially explore the word embedding attack setting, by describing our attack strategy based on the words present in the input, and how we can cleverly modify these words to misclassify the input. We will also explore the poisoning attack, where we change word embedding representation of certain words to poison the model and misclassify targeted inputs. We will present the attack accuracies in different downstream student tasks and how they differ based on the different attack parameters. This will be followed by the details of the attack strategy for the sentence embedding model and how we take the feature of input sentences like length into account to attack the model. The words are also an important feature for sentence embedding but the output of the embedding is dependent on other factors as well, like the context of word etc. We then report the attack accuracy for the attacks based on sentence embedding teacher model. The rest of the paper is followed by an discussion on the finding and some how the traditional defense techniques are not effective against our attack strategies.

==> sent_acc.tikz.tex <==
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.75,0.75,0}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xlabel={Number of real sentences added},
xmin=-0.95, xmax=19.95,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Accuracy},
legend style={at={(0.75,0.55)},anchor=north},
ymin=59.05, ymax=101.95,
ytick style={color=black}
]
\addplot [semithick, color0, mark=triangle*, mark size=3, mark options={solid}]
table {%
0 100
1 99
2 98
3 97
4 97
5 98
6 96
7 85
8 79
9 76
10 76
11 75
12 74
13 70
14 68
15 68
16 65
17 63
18 61
19 61
};
\addlegendentry{Accuracy}
\end{axis}

\begin{axis}[
axis y line=right,
tick align=outside,
x grid style={white!69.01960784313725!black},
xmin=-0.95, xmax=19.95,
xtick pos=left,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={Dot Product from real sample},
ymin=0.85, ymax=0.96,
legend style={at={(0.75,0.665)},anchor=north},
ytick pos=right,
ytick style={color=black}
]
\addplot [semithick, blue, mark=*, mark size=3, mark options={solid}]
table {%
0 0.86
1 0.869
2 0.86
3 0.866
4 0.889
5 0.894
6 0.889
7 0.898
8 0.907
9 0.93
10 0.929
11 0.935
12 0.938
13 0.942
14 0.944
15 0.948
16 0.948
17 0.954
18 0.956
19 0.955
};
\addlegendentry{Dot Prod}
\end{axis}

\end{tikzpicture}
